Signature-based validation of real-world economic scenarios

Motivated by insurance applications, we propose a new approach for the validation of real-world economic scenarios. This approach is based on the statistical test developed by Chevyrev and Oberhauser (2022) and relies on the notions of signature and maximum mean distance. This test allows to check whether two samples of stochastic processes paths come from the same distribution. Our contribution is to apply this test to a variety of stochastic processes exhibiting different pathwise properties (H{\"o}lder regularity, autocorrelation, regime switches) and which are relevant for the modelling of stock prices and stock volatility as well as of inflation in view of actuarial applications.

==> bibli.tex <==
\bibliographystyle{plainnat}
\begin{thebibliography}{99}\footnotesize
    {}
    \bibitem[Asadi et~al.(2020)]{asadi2020}
    Asadi, S. and Al Janabi, M. A. M. (2020). Measuring market and credit risk under
    {S}olvency {II}: evaluation of the standard technique versus internal models for stock
    and bond markets. In: \emph{Eur. Actuar. J.} 10.2, pp. 425-456.
    {}
    \bibitem[Black and Scholes(1973)]{black1973pricing}
    Black, F. and Scholes, M. (1973). The pricing of options and corporate liabilities. In:
    \emph{J. Polit. Econ.} 81.3, pp. 637-654.
    {}
    \bibitem[Boedihardjo et~al.(2016)]{boedihardjo2016signature}
    Boedihardjo, H., Geng, X., Lyons, T., and Yang, D. (2016). The signature of a rough
    path: uniqueness. In: \emph{Adv. Math.} 293, pp. 720-737.
    {}
    \bibitem[Boudreault and Panneton(2009)]{boudreault2009}
    Boudreault, M. and Panneton, C.-M. (2009). Multivariate models of equity returns for
    investment guarantees valuation. In: \emph{N. Am. Actuar. J.} 13.1, pp. 36-53.
    {}
    \bibitem[Buehler et~al.(2020)]{buehler2020generating}
    Buehler, H., Horvath, B., Lyons, T., Perez Arribas, I., and Wood, B. (2020). Generating
    financial markets with signatures. In: \emph{Available at SSRN 3657366}.
    {}
    \bibitem[Chen(1957)]{chen1957}
    Chen, K.-T. (1957). Integration of paths, geometric invariants and a generalized
    {B}aker-{H}ausdorff formula. In: \emph{Ann. of Math. (2)} 65, pp. 163-178.
    {}
    \bibitem[Chevyrev and Kormilitzin(2016)]{chevyrev2016primer}
    Chevyrev, I. and Kormilitzin, A. (2016). A primer on the signature method in machine
    learning. In: \emph{arXiv preprint arXiv:1603.03788}.
    {}
    \bibitem[Chevyrev and Lyons(2016)]{chevyrev2016characteristic}
    Chevyrev, I. and Lyons, T. (2016). Characteristic functions of measures on geometric
    rough paths. In: \emph{Ann. Probab.} 44.6, pp. 4049-4082.
    {}
    \bibitem[Chevyrev and Oberhauser(2022)]{chevyrev2018signature}
    Chevyrev, I. and Oberhauser, H. (2022). Signature moments to characterize laws of
    stochastic processes. In: \emph{Journal of Machine Learning Research} 23.176, pp. 1-42.
    {}
    \bibitem[Cuchiero et~al.(2022)]{cuchiero2022signature}
    Cuchiero, C., Gazzani, G., and Svaluto-Ferro, S. (2022). Signature-based models: theory
    and calibration. In: \emph{arXiv preprint arXiv:2207.13136}.
    {}
    \bibitem[Cucker and Smale(2002)]{cucker2002}
    Cucker, F. and Smale, S. (2002). On the mathematical foundations of learning. In:
    \emph{Bull. Amer. Math. Soc. (N.S.)} 39.1, pp. 1-49.
    {}
    \bibitem[Dudley(2022)]{dudley2002real}
    Dudley, R. M. (2002). \emph{Real analysis and probability}. Vol. 74. Cambridge Studies
    in Advanced Mathematics. Revised reprint of the 1989 original. Cambridge University
    Press, Cambridge, pp. x+555.
    {}
    \bibitem[Fawcett(2002)]{fawcett2002problems}
    Fawcett, T. (2002). Problems in stochastic analysis: Connections between rough paths
    and non-commutative harmonic analysis. PhD thesis. University of Oxford.
    {}
    \bibitem[Fermanian(2021)]{fermanian2021embedding}
    Fermanian, A. (2021). Embedding and learning with signatures. In: \emph{Comput.
    Statist. Data Anal.} 157, Paper No. 107148, 23.
    {}
    \bibitem[Floryszczak et~al.(2019)]{floryszczak2019}
    Floryszczak, A., Lévy Véhel, J., and Majri, M. (2019). A conditional equity risk model
    for regulatory assessment. In: \emph{Astin Bull.} 49.1, pp. 217-242.
    {}
    \bibitem[Friz and Victoir(2010)]{friz2010multidimensional}
    Friz, P. K. and Victoir, N. B. (2010). \emph{Multidimensional stochastic processes as
    rough paths}. Vol. 120. Cambridge Studies in Advanced Mathematics. Theory and
    applications. Cambridge University Press, Cambridge, pp. xiv+656.
    {}
    \bibitem[Gatheral et~al.(2018)]{gatheral2018volatility}
    Gatheral, J., Jaisson, T., and Rosenbaum, M. (2018). Volatility is rough. In:
    \emph{Quant. Finance} 18.6, pp. 933-949.
    {}
    \bibitem[Graf et~al.(2014)]{graf2014}
    Graf, S., Haertel, L., Kling, A., and Ruÿ, J. (2014). The impact of inflation risk on
    financial planning and risk-return profiles. In: \emph{Astin Bull.} 44.2, pp. 335-365.
    {}
    \bibitem[Gretton et~al.(2012)]{gretton2012kernel}
    Gretton, A., Borgwardt, K. M., Rasch, M. J., Schölkopf, B., and Smola, A. (2012). A
    kernel two-sample test. In: \emph{J. Mach. Learn. Res.} 13, pp. 723-773.
    {}
    \bibitem[Gretton et~al.(2009)]{gretton2009fast}
    Gretton, A., Fukumizu, K., Harchaoui, Z., and Sriperumbudur, B. K. (2009). A fast,
    consistent kernel two-sample test. In: \emph{Advances in neural information processing
    systems} 22.
    {}
    \bibitem[Gyurkó and Lyons(2010)]{gyurko2010}
    Gyurkó, L. G. and Lyons, T. (2010). Rough paths based numerical algorithms in
    computational finance. In: \emph{Mathematics in finance}. Vol. 515. Contemp. Math.
    Amer. Math. Soc., Providence, RI, pp. 17-46.
    {}
    \bibitem[Gyurkó et~al.(2013)]{gyurko2013extracting}
    Gyurkó, L. G., Lyons, T., Kontkowski, M., and Field, J. (2013). Extracting information
    from the signature of a financial data stream. In: \emph{arXiv preprint
    arXiv:1307.7244}.
    {}
    \bibitem[Hambly and Lyons(2010)]{hambly2010uniqueness}
    Hambly, B. and Lyons, T. (2010). Uniqueness for the signature of a path of bounded
    variation and the reduced path group. In: \emph{Ann. of Math. (2)} 171.1, pp. 109-167.
    {}
    \bibitem[Hardy et~al.(2006)]{hardy2006}
    Hardy, M. R., Freeland, R. K., and Till, M. C. (2006). Validation of long-term equity
    return models for equity-linked guarantees. In: \emph{N. Am. Actuar. J.} 10.4,
    pp. 28-47.
    {}
    \bibitem[Johnson et~al.(1994)]{johnson1994}
    Johnson, N. L., Kotz, S., and Balakrishnan, N. (1994). \emph{Continuous univariate
    distributions. {V}ol. 1}. Second. Wiley Series in Probability and Mathematical Statistics:
    Applied Probability and Statistics. A Wiley-Interscience Publication. John Wiley \&
    Sons, Inc., New York, pp. xxii+756.
    {}
    \bibitem[Levin et~al.(2013)]{levin2013learning}
    Levin, D., Lyons, T., and Ni, H. (2013). Learning from the past, predicting the statistics
    for the future, learning an evolving system. In: \emph{arXiv preprint arXiv:1309.0260}.
    {}
    \bibitem[Liao et~al.(2019)]{liao2019learning}
    Liao, S., Lyons, T., Yang, W., and Ni, H. (2019). Learning stochastic differential
    equations using RNN with log signature features. In: \emph{arXiv preprint
    arXiv:1908.08286}.
    {}
    \bibitem[Lin and Yang (2020)]{lin2020}
    Lin, X. S. and Yang, S. (2020). Efficient dynamic hedging for large variable annuity
    portfolios with multiple underlying assets. In: \emph{Astin Bull.} 50.3, pp. 913-957.
    {}
    \bibitem[Lyons(1998)]{lyons1998}
    Lyons, T. (1998). Differential equations driven by rough signals. In: \emph{Rev. Mat.
    Iberoamericana} 14.2, pp. 215-310.
    {}
    \bibitem[Lyons et~al.(2007)]{lyons2007differential}
    Lyons, T., Caruana, M., and Lévy, T. (2007). \emph{Differential equations driven by
    rough paths}. Vol. 1908. Lecture Notes in Mathematics. Lectures from the 34th Summer
    School on Probability Theory held in Saint-Flour, July 6-24, 2004, With an introduction
    concerning the Summer School by Jean Picard. Springer, Berlin, pp. xviii+109.
    {}
    \bibitem[Morrill et~al.(2020)]{morrill2020generalised}
    Morrill, J., Fermanian, A., Kidger, P., and Lyons, T. (2020). A generalised signature
    method for multivariate time series feature extraction. In: \emph{arXiv preprint
    arXiv:2006.00873}.
    {}
    \bibitem[Ni et~al.(2021)]{ni2021sig}
    Ni, H., Szpruch, L., Sabate-Vidales, M., Xiao, B., Wiese, M., and Liao, S. (2021).
    Sig-Wasserstein GANs for time series generation. In: \emph{Proceedings of the Second
    ACM International Conference on AI in Finance}, pp. 1-8.
    {}
    \bibitem[Otero et~al.(2012)]{otero2012estimating}
    Otero, L., Durán, P., Fernández, S., and Vivel, M. (2012). Estimating insurers capital
    requirements through Markov switching models in the Solvency II framework. In:
    \emph{International Research Journal of Finance and Economics} 86, pp. 20-38.
    {}
    \bibitem[Oxford-Man Institute of Quantitative Finance (2023)]{Realized_Vol_Data}
    Oxford-Man Institute of Quantitative Finance (2023). \emph{Realized Library}. \url
    {https://www.oxford-man.ox.ac.uk/research/realized-library/}. Accessed on: 2023-01-27.
    {}
    \bibitem[Perez Arribas(2020)]{perez2020signatures}
    Perez Arribas, I. (2020). Signatures in machine learning and finance. PhD thesis.
    University of Oxford.
    {}
    \bibitem[Sen(1977)]{kumar1977}
    Sen, P. K. (1977). Almost sure convergence of generalized {$U$}-statistics. In:
    \emph{Ann. Probability} 5.2, pp. 287-290.
    {}
    \bibitem[Smith(1985)]{smith1985numerical}
    Smith, G. D. (1985). \emph{Numerical solution of partial differential equations}. Third.
    Oxford Applied Mathematics and Computing Science Series. Finite difference methods.
    The Clarendon Press, Oxford University Press, New York, pp. xiv+337.
    {}
    \bibitem[U.S. Bureau of Labor Statistics (2023)]{BLS_Inflation_Data}
    U.S. Bureau of Labor Statistics (2023). \emph{Consumer Price Index for All Urban
    Consumers, U.S. city average, All items}. \url {https://www.bls.gov/cpi/data.htm}.
    Accessed on: 2023-01-27.
    {}
    \bibitem[Wang et~al.(2019)]{wang2019estimation}
    Wang, X., Xiao, W., and Jun, Y. (2019). Estimation and Inference of fractional
    continuous-time model with discrete-sampled data. In: \emph{SMU Economics and
    Statistics Working Paper Series, Paper No. 17-2019}.
    {}
    \bibitem[Young(1936)]{young1936}
    Young, L. C. (1936). An inequality of the {H}ölder type, connected with {S}tieltjes
    integration. In: \emph{Acta Math.} 67.1, pp. 251-282.
    {}
    \bibitem[Zhu et~al.(2019)]{zhu2018}
    Zhu, X., Hardy, M. R., and Saunders, D. (2018). Dynamic hedging strategies for cash
    balance pension plans. In: \emph{Astin Bull.} 48.3, pp. 1245-1275.
\end{thebibliography}

